Test-Time Training with Masked Autoencoders

Test-time training adapts to a new test distribution on the fly by optimizing a model for each test input using self-supervision. In this paper, we use masked autoencoders for this one-sample learning problem. Empirically, our simple method improves generalization on many visual benchmarks for distribution shifts. Theoretically, we characterize this improvement in terms of the bias-variance trade-off.

==> tex/intro_1.tex <==
\section{Introduction}
Generalization from labeled training data to new test data is the central theme of supervised learning, and a hallmark of intelligence.
Deep learning generalizes well when the training and test data are from the same distribution, but struggles when they are different, for example, in visual appearance.
Generalization of state-of-the-art models suffers significantly even under seemingly minor distribution shifts that barely affect humans.

How to generalize to new test distributions unknown during training?
The naturally revealed test input provides a clue about the test distribution where it is sampled.
Test-time training~\cite{sun2020test, hansen2020self, banerjee2021self, sun2021online}
is a paradigm of methods that formulates each test input into a one-sample learning problem, before making a prediction on this input itself.
Each prediction is made not only from a different input, but also by a different model.

Since the test input comes without ground truth label, learning signal must be provided through self-supervision.
Prior work \cite{sun2020test} uses rotation prediction, which hopes to form semantic features by learning the orientation of rotated images. 
For natural scenes, image rotation can be trivially predicted, without scene understanding, from the horizon's orientation alone.
Even for centered objects, many classes, e.g. frogs and lizards, have mostly top-down views, for which every orientation looks equally plausible.
In both cases, rotation prediction is unlikely to form semantic features as hoped for.
This lacks generality...
% If the lack of generality seems harmful to supervised learning, it is only worse for generalizing to truly unknown distributions.
 
Latest advances in self-supervised learning suggest masked autoencoding as a potentially general-purpose task.
This task is simple: remove parts of the data, and predict the removed content.
In natural language processing, masked autoencoding \cite{devlin2018bert} and the closely related task of autoregressive language modeling \cite{mikolov2013efficient, radford2018improving, brown2020language}
have long been a staple of the community. 
Recent research in computer vision also shows that predicting missing patches on images can lead to state-of-the-art performance on a variety of downstream tasks and datasets \cite{mae, beit, simmim}.

Motivated by these successes, we experiment with masked autoencoding (MAE) as self-supervision for test-time training on four datasets.
Our method leads to improvements in all of them.
We also theoretically characterize the relationship between our method and the well known bias-variance trade-off in statistics.

==> tex/intro_2.tex <==
\section{Introduction}
Generalization from labeled training data to unlabeled test data is the central theme of supervised learning, and a hallmark of intelligence.
While most of the research focuses on generalization when the training and test data are drawn from the same distribution, this is rarely the case for real world deployment~\cite{torralba2011unbiased}, and is certainly not true for environments where intelligence has emerged.

Generalization to new test distributions requires new assumptions.
What are fundamental assumptions behind the wide range of distributions in the world?
This is understandably a hard problem, and it is even harder to design such priors into model architectures and training process, as attempted by most papers in this area
\cite{imagenet_c, geirhos2018generalisation, vasiljevic2016examining}.

The success of artificial intelligence today is about turning hard design problems into learning problems.
In our case, each test input itself offers one piece of data, from the test distribution, to form a learning problem.
This is the key insight behind test-time training~\cite{sun2020test, luo2020consistent, banerjee2021self, hansen2020self}.
Because this input is unlabeled, learning can only be performed with self-supervision.
The assumption here, therefore, is that the self-supervised task produces useful features for the main task on the test distributions.

What self-supervised task would be general enough to satisfy this assumption?
We propose the use of masked autoencoding.
This task is simple: remove parts of the data, and predict the removed content.
In natural language processing, masked autoencoding \cite{devlin2018bert} and the closely related task of autoregressive language modeling \cite{mikolov2013efficient, radford2018improving, brown2020language} have long been a staple of the community.
Also with a long history in computer vision \cite{efros1999texture, pathak2016context}, masked autoencoding has recently shown state-of-the-art performance on a variety of downstream tasks and datasets \cite{mae, beit, simmim}.

We experiment with masked autoencoding as self-supervision for test-time training on four datasets.
Our method leads to improvements in all of them.
Our prove that test-time training with autoencoding helps a linear model under distribution shifts,
revealing more intuition for why our method works from a theoretical perspecitve.
\footnote{The code and the models will be made public upon acceptance.}


==> tex/intro_3.tex <==
\section{Introduction}
Generalization from labeled training data to unlabeled test data is the central theme of supervised learning, and a hallmark of intelligence.
While most of the research focuses on generalization when the training and test data are drawn from the same distribution, this is rarely the case for real world deployment~\cite{torralba2011unbiased}, and is certainly not true for environments where intelligence has emerged.

% Because there is no training data from the new test distribution, most algorithms try to guess what this new distribution is about.
% This is very hard.
% But there is in fact one piece of data from the test distribution
% -- the test input itself.
% This is the key insight of test-time training 
% \cite{sun2020test, luo2020consistent, hansen2020self, banerjee2021self}
% which produces a different model for each test input by first using it for training.

% The problem of generalizing to a new test distribution is hard because most models today are fixed during deployment, even when the test distribution changes \cite{imagenet_c, geirhos2018generalisation, vasiljevic2016examining}.

What makes generalizing to a novel distribution hard is 

How to generalize to a new test distribution, when we do not have data from it during training?
Each test input itself is one piece of data from the test distribution, thus provides the most relevant learning signals.
This is the key insight of test-time training 
\cite{sun2020test, luo2020consistent, hansen2020self, banerjee2021self}
which produces a different model for each test input by first using it for training.

How to train on a test input without label?
Self-supervision!
Test-time training relies on a self-supervised task that produces useful features for the main task on a wide range of test distributions.
We propose the use of masked autoencoding: 
remove parts of the data, and predict the removed content.
In natural language processing, masked autoencoding \cite{devlin2018bert} and the closely related task of autoregressive language modeling \cite{mikolov2013efficient, radford2018improving, brown2020language} have long been a staple of the community.
Also with a long history in computer vision \cite{efros1999texture, pathak2016context}, masked autoencoding has recently shown state-of-the-art performance on a variety of downstream tasks and datasets \cite{mae, beit, simmim}.

We experiment with masked autoencoding as self-supervision for test-time training on four datasets.
Our method leads to improvements in all of them.
Our prove that test-time training with autoencoding helps a linear model under distribution shifts,
revealing more intuition for why our method works from a theoretical perspecitve.
\footnote{The code and the models will be made public upon acceptance.}


==> tex/related_old.tex <==
\section{Related Work}
\label{related}

\subsection{Masked Autoencoders and Self-Supervised Learning}
\label{related-mae}
Key to the success of deep learning is the formation of semantic features that transfer across many tasks.
The goal of self-supervised pre-training is to learn these transferable features without human annotations, by making up inputs and labels to an auxiliary pretext task.
Given an original input image $x$, the pretext task of masked autoencoding \cite{mae} splits the image into many (e.g. 196) non-overlapping patches, randomly masks out majority of the patches (e.g. 75\%), and trains a model to reconstruct the missing ones by optimizing the mean squared error between the original and reconstructed pixels.

This model, called a masked autoencoder (MAE), is composed of two parts: a large encoder and a small decoder, both based on Vision Transformers \cite{dosovitskiy2020image}.
For a downstream task such as object recognition, the encoder takes in all the image patches and outputs their features, which then become input to a task-specific linear projection head.
There are two common ways to combine the pre-trained encoder and untrained head.
1) Fine-tuning: both the encoder and head are trained, end-to-end, for the downstream task.
2) Linear probing: the encoder is frozen as a fixed feature extractor, and only the head is trained.
We refer back to these training options in Section \ref{method} in the context of our method.

\subsection{Generalization under Distribution Shifts}
\label{related-generalization}
% Traditionally, training and test data are drawn i.i.d. from the same distribution; 
% deep learning generalizes well by interpolating the training set with rather limited prior knowledge \cite{zhang2021understanding}.
When training and test distributions are different, generalization is intrinsically hard. 
% since interpolation cannot cover many of the test samples \cite{recht2018cifar, recht2019imagenet, shankar2019systematic, dodge2017study}.
% One way to turn extrapolation into interpolation again is to make the training distribution wider, and the training set larger, to cover the test distribution.
% This brute force approach, however, naturally falls short of scaling up to all possible distribution shifts in the world, even if they could be anticipated at training time.
Training on many distribution shifts at once causes underfitting \cite{zheng2016improving, dodge2017quality}.
The robustness obtained by training or fine-tuning on one type of distribution shift (e.g. Gaussian noise) also does not transfer to another (e.g. salt-and-pepper noise) \cite{geirhos2018generalisation, vasiljevic2016examining}, even for visually similar corruptions.

To avoid the hardness of extrapolation, researchers work on alternative problem settings that anticipate the test distribution.
For domain generalization \cite{li2018deep, li2019episodic, shankar2018generalizing, muandet2013domain, carlucci2019domain, ghifary2015domain, mahajan2021domain, gulrajani2020search},
a meta distribution generates many distribution shifts, some of which are used for training and others for testing.
For domain adaptation \cite{long2015learning, long2016unsupervised, csurka2017domain, chen2011co, sun2019uda, hoffman2017cycada, chen2018adversarial, gong2012geodesic}, 
a potentially unlabeled dataset from the test distribution is available for training.
Solutions motivated by these settings share the same flaw as augmenting the training set:
they are only effective on the particular meta / test distribution that they were trained for.

% Supervised learning evaluates generalization on each test input independently, even when using a test set to statistically approximate the population mean, reflecting that in practice test data might not come from the same distribution.
% To follow this protocol, test-time training needs to formulate a single-input learning problem, without relying on other test data.
% The single test input also comes without ground truth label, so learning signal can only be provided through self-supervision.

\subsection{Test-Time Training}
\label{related-ttt}
% An alternative to this one-model-fits-all philosophy is ,
% which trains a different model for each test input during deployment,
% immediately before making a prediction on it.

% Most algorithms today \cite{imagenet_c, geirhos2018generalisation, vasiljevic2016examining} train a fixed model for all distributions that will be encountered during deployment.
% This makes it is hard to find general priors that integrate into training and model design.

Test-time training (TTT) \cite{sun2020test} is a paradigm of methods that generalizes to distribution shifts without anticipating them, through self-supervised learning on each test input $x$.
In \cite{sun2020test}, the main task is object recognition, and the self-supervised task is rotation prediction \cite{gidaris2018unsupervised}: $x$ is simply rotated in the image plane by multiples of 90 degrees to create a four-way classification problem.

The network for TTT is Y-shaped: a feature extractor $f$, followed simultaneous by a self-supervised head $g$ and a main task head $h$.
During training, labels are available for both the self-supervised task, using $g\circ f$, and the main task, using $h\circ f$; so both branches are trained jointly by summing their losses together for gradient descent.
During testing, for each $x$, only the self-supervised task is labeled;
% \ygc{maybe replace with something in the spirit of - the model utilizes the "free" labels of the self supervised task}
so $g\circ f$ is trained, end-to-end, on this single input.
This produces a different model, call it $f_x$ (and $g_x$), 
initialized from $f$ (and $g$), locally optimized for each test input $x$. 
After making a prediction on $x$, now with $h\circ f_x$, the algorithm never uses $f_x$ (and $g_x$) again;
the entire process repeats itself for the next input, again initializing from the old $f$ (and $g$).

% Prior work \cite{sun2020test} uses rotation prediction, which hopes to form semantic features by learning the orientation of rotated images. 
% For natural scenes, image rotation can be trivially predicted, without scene understanding, from the horizon's orientation alone.
% Even for centered objects, many classes, e.g. frogs and lizards, have mostly top-down views, for which every orientation looks equally plausible.
% In both cases, rotation prediction is unlikely to form semantic features as hoped for.
% This lacks generality...
% If the lack of generality seems harmful to supervised learning, it is only worse for generalizing to truly unknown distributions.

TTT as explained above is not a new problem setting; it is a proposed solution to the canonical problem of generalization.
% It strictly follows the protocol of so-called zero-shot generalization.
% Besides the rather exposed and standard priors in the self-supervised task, 
% TTT does not rely on any information about the test distribution, 
% until it is unavoidably revealed by only one sample.
Our paper stay in the same setting. 
Other followups have worked on new settings such as
% an online stream of samples from similar distributions, and 
a batch \cite{wang2020tent} or dataset \cite{liu2021ttt++} of samples from the test distribution.

Before \cite{sun2020test}, single-image training has been performed for super-resolution \cite{shocher2018zero}.
The philosophy of TTT is also preceded by that of local learning \cite{bottou1992local} and transductive learning \cite{vapnik2013nature}, although usually performed for support vector machines with multiple test samples \cite{collobert2006large, joachims2002learning}.
Since \cite{sun2020test}, TTT has been applied to many fields with domain-specific self-supervised tasks:
vision-based reinforcement learning \cite{hansen2020self}, 
model-based legged locomotion \cite{sun2021online},
tracking objects in videos \cite{fu2021learning},
natural language question answering \cite{banerjee2021self},
and even medical imaging \cite{karani2021test}.


==> tex/trash.tex <==
\begin{table}
\footnotesize
  \centering
  \label{tab:lin_prob}
  \setlength\tabcolsep{2.5pt}
  \begin{tabular}{l|cccccccccccccccccc}
    \toprule
    & brigh & cont & defoc & elast & fog & frost & gauss & glass & impul & jpeg & motn & pixel & shot & snow & zoom\\
    \midrule
    Probing & 59.8 & 4.8 & 16.9 & 24.6 & 28.6 & 29.2 & 10.5 & 13.8 & 11.2 & 38.3 & 20.0 & 34.4 & 11.0 & 22.6 & 24.3\\
TTT-MAE & 32.5 & 6.2 & 12.2 & 19.4 & 15.8 & 23.1 & 12.1 & 12.4 & 13.3 & 23.9 & 11.6 & 16.7 & 12.8 & 12.1 & 15.9\\
    \bottomrule
  \end{tabular}
  \vspace{1ex}
  \caption{\textbf{Linear probing}}
\end{table}

\begin{table}
\footnotesize
  \centering
  \label{tab:vit_rotation_vit_reconstruction}
  \setlength\tabcolsep{3.pt}
  \begin{tabular}{l|cccccccccccccccccc}
    \toprule
    & brigh & cont & defoc & elast & fog & frost & gauss & glass & impul & jpeg & motn & pixel & shot & snow & zoom\\
    \midrule
Base rot. & 56.3 & 23.2 & 20.5 & 34.1 & 18.1 & 24.7 & 9.7 & 13.0 & 9.1 & 37.1 & 19.0 & 20.6 & 11.7 & 22.1 & 23.5 \\
TTT rot. &  37.9 & 7.8 & 9.2 & 26.4 & 10.7 & 13.5 & 6.0 & 9.0 & 6.2 & 27.4 & 11.6 & 15.4 & 6.9 & 10.2 & 15.1 \\
    \bottomrule
  \end{tabular}
  \vspace{1ex}
  \caption{\textbf{Joint training Rotation results with ViT architecture.} \ygc{The details: we trained a ViT-Small model with ViT-Small head for 20 epochs jointly. We than TTT it for 5 steps on a minimized version of Imagenet-Val (the same one with each augmentation). We could not make it work unfortunately, probably due to the size of the model (73.45M Params). We basically could not make it work and this is what we should argue here.} }
\end{table}

\subsection{CheXpert Results}
CheXpert dataset contains 224,316 chest radiographs of 65,240 patients with both frontal and lateral views available. Each single-view chest image is annotated with 5 medical observations, age and sex. The data divided into X training images and Y test images. 

To evaluate our model on real-world distribution shifts, we first split the training data and the test data into two age categories (above 65 and bellow 55). We then train a classifier on one split of the training data to predict the gender of the patent. Finally, we compare our model performance on the second split of the test data. \ygc{currently don't have good results to share. will have in a day}


\begin{table}[t!]
  \centering
  \label{tab:portraits_results}
  \begin{tabular}{l|l|c|c|c}
    \toprule
    Train split & Test split & Test size & Baseline & TTT (20 steps) \\
    \midrule
    $\leq$ 1940  & $\geq$ 1970 & 21,439 & 75.42 & \textbf{76.81} \\
    $\geq$ 1970  & $\leq$ 1940 & 3,820 & 87.28 & \textbf{87.54}  \\
    \bottomrule
  \end{tabular}
  \vspace{1ex}
  \caption{\textbf{Results on the portrait dataset.}}
\end{table}
